Equivariant Learning of Stochastic Fields: Gaussian Processes and Steerable Conditional Neural Processes

Motivated by objects such as electric fields or fluid streams, we study the problem of learning stochastic fields, i.e. stochastic processes whose samples are fields like those occurring in physics and engineering. Considering general transformations such as rotations and reflections, we show that spatial invariance of stochastic fields requires an inference model to be equivariant. Leveraging recent advances from the equivariance literature, we study equivariance in two classes of models. Firstly, we fully characterise equivariant Gaussian processes. Secondly, we introduce Steerable Conditional Neural Processes (SteerCNPs), a new, fully equivariant member of the Neural Process family. In experiments with Gaussian process vector fields, images, and real-world weather data, we observe that SteerCNPs significantly improve the performance of previous models and equivariance leads to improvements in transfer learning tasks.

==> math.tex <==
\def\inv{^{-1}}

\def\R{\mathbb{R}}
\def\X{\mathcal{X}}
\def\Y{\mathcal{Y}}
\def\N{\mathcal{N}}

\def\grp{G}
\def\op{\cdot}

\def\GP{\mathcal{GP}}

\def\x{\mathbf{x}}


\newtcbtheorem[auto counter]{proposition}{Proposition}{
    lower separated=false,
    colback=oxverylightblue,
    colframe=oxlightgrey,
    colbacktitle=oxvlightgrey,
    coltitle=black,
    arc=0mm,
    enhanced,
    boxed title style={colframe=oxlightgrey},
    attach boxed title to top left={xshift=0.3cm,yshift=-2mm},
}{def}

\newtcbtheorem[auto counter]{theorem}{Theorem}{
    lower separated=false,
    colback=oxverylightblue,
    colframe=oxlightgrey,
    colbacktitle=oxvlightgrey,
    coltitle=black,
    arc=0mm,
    enhanced,
    boxed title style={colframe=oxlightgrey},
    attach boxed title to top left={xshift=0.3cm,yshift=-2mm},
}{def}

==> poster_sections/equiv_deepsets.tex <==
We can characterise all functions of the form 
\begin{align*}
    Z \mapsto f_Z \quad \text{subject to} \quad f_{g \op Z}(x) = \rho(r) f_Z(g\inv \op x)
\end{align*}
These are functions that take some set of points, and produce a \textit{field}, i.e. a function that can be evaluated anywhere. Any such function can be expressed as
\begin{align*}
     f_Z = D \left( \sum_{i=1}^n K(\cdot, x_i) \begin{bmatrix} y_i \\ 1 \end{bmatrix} \right) \quad \text{subject to} \quad \begin{cases} K \text{ is an equivariant kernel} \\ D \text{ is an equivariant map between fields} \end{cases}
\end{align*}

==> poster_sections/equivariant_gps.tex <==
\begin{theorem}{}{}
    \label{thm:equivgp}
    A Gaussian process $\GP(\mathbf{m},K)$ is $G$-invariant, equivalently the posterior $G$-equivariant, if and only if
    \begin{enumerate}[noitemsep]
        \item For all $\mathbf{x} \in\R^n$, $g \in \grp$, 
        \begin{enumerate}[noitemsep]
            \item $\mathbf{m}(\mathbf{x})=\mathbf{m}$
            \item $\rho(r)\mathbf{m}=\mathbf{m}$
        \end{enumerate}
        \item For all $\mathbf{x},\mathbf{x}'\in\R^n$, $g \in \grp$
        \begin{enumerate}[noitemsep]
            \item $K(\mathbf{x},\mathbf{x}')=K(\mathbf{x}-\mathbf{x}', \mathbf{0}) := \hat{K}(\x - \x')$
            \item $K(r \op \x, r \op \x') = \rho(h) K(\x, \x')\rho(r)\inv$
        \end{enumerate}
    \end{enumerate}
\end{theorem}
\vspace{-1.2em}
\begin{center}
    \def\width{0.2}
    \hspace{4em}
    \includegraphics[width=\width\linewidth]{Pictures/illustrations/sample_rbf.pdf}
    \hfill
    \includegraphics[width=\width\linewidth]{Pictures/illustrations/sample_div_free.pdf}
    \hfill
    \includegraphics[width=\width\linewidth]{Pictures/illustrations/sample_curl_free.pdf}
    \hspace{4em}
    \vspace{-1em}
    \captionof{figure}{Example RBF, divergence free, and curl free equivariant Guassian Processes}
\end{center}
\vspace{-2em}

==> poster_sections/experiments_era5.tex <==
{
\scriptsize
\begin{tabular}[b]{lrr}
    \toprule
    \textbf{Model} & US & China  \\
    \midrule
    GP & 0.386$\pm$0.005& -0.755$\pm$0.001\\
    CNP    & 0.001$\pm$0.017& -2.456$\pm$0.365 \\
    ConvCNP & 0.898$\pm$0.045& -0.890$\pm$0.059\\
    \midrule
    %SteerCNP ($SO(2)$)&0.598$\pm$0.022&-4.680$\pm$0.552\\
    SteerCNP ($C_4$)       & \textbf{1.255}$\pm$0.019& -0.578$\pm$0.173\\
    SteerCNP ($C_{8}$)    & 1.038$\pm$0.026& -0.582$\pm$0.104\\
    SteerCNP ($C_{16}$)    & 1.094$\pm$0.015& -0.550$\pm$0.073\\
    SteerCNP ($D_4$)       & 1.037$\pm$0.037& \textbf{-0.429}$\pm$0.067 \\
    SteerCNP ($D_8$)     & 1.032$\pm$0.011& -0.539$\pm$0.129\\
    \bottomrule
\end{tabular}
}
\vspace{-1em}
\captionof{table}{Weather completion results}
\vspace{-0.5em}

\tcblower

\includegraphics[width=\linewidth]{Pictures/illustrations/ERA5_us_half.pdf}
\vspace{-2.5em}
\captionof{figure}{Example region and wind map}
\vspace{-0.5em}


==> poster_sections/experiments_mnist.tex <==
{
    \scriptsize
    \begin{tabular}{lrrr}
        \toprule
        \textbf{Train dataset} &                   \multicolumn{1}{l}{MNIST} &                \multicolumn{1}{l}{rotMNIST} &                   \multicolumn{1}{r}{MNIST} \\
        \textbf{Test dataset} & \multicolumn{1}{l}{MNIST} &\multicolumn{1}{l}{MNIST} &  {extMNIST} \\
        \textbf{Model}            &                         &                         &                      \\
        \midrule
        GP                 &         {0.39$\pm$0.30} &         {0.39$\pm$0.30} &         {0.72$\pm$0.17} \\
        CNP                &         {0.76$\pm$0.05} &         {0.66$\pm$0.06} &        {-1.11$\pm$0.06} \\
        ConvCNP            &         {1.01$\pm$0.01} &         {0.95$\pm$0.01} &         {1.08$\pm$0.02} \\
        \midrule
        SteerCNP($C_4$)    &         {1.05$\pm$0.02} &  \textbf{1.02$\pm$0.03} &         {1.14$\pm$0.02} \\
        SteerCNP($C_{8}$)  &  \textbf{1.07$\pm$0.03} &  \textbf{1.05$\pm$0.04} &  \textbf{1.16$\pm$0.03} \\
        SteerCNP($C_{16}$) &  \textbf{1.08$\pm$0.03} &  \textbf{1.04$\pm$0.03} &  \textbf{1.17$\pm$0.05} \\
        SteerCNP($D_4$)    &  \textbf{1.08$\pm$0.03} &  \textbf{1.05$\pm$0.03} &         {1.14$\pm$0.03} \\
        SteerCNP($D_8$)    &  \textbf{1.08$\pm$0.03} &  \textbf{1.04$\pm$0.04} &  \textbf{1.17$\pm$0.02} \\
        \bottomrule
    \end{tabular}
}
\vspace{-1em}
\captionof{table}{MNIST completion results}
\vspace{-0.5em}

\tcblower

\includegraphics[width=0.95\linewidth]{Pictures/illustrations/train_rotation.pdf}
\vspace{-1em}
\captionof{figure}{Example inferences}
\vspace{-0.5em}

==> poster_sections/motivation.tex <==
\textbf{Scalar} valued stochastic processes are well studied, i.e. random functions
\begin{align*}
    f: \X \to \R \text{ or even } f:\X \to \R^n
\end{align*}
If we want to model functions whose outputs are \textbf{vector} valued, or higher-order tensors, we can still model these as functions 
\begin{align*}
    f:\X \to \R^n
\end{align*}
but we have the additional baggage of choosing a \textbf{basis} to be able to represent the vector values as a series of scalars.
\begin{multicols}{2}
\begin{itemize}[noitemsep]
    \item Choice of basis is arbitrary
    \item[$\implies$] Shouldn't affect our inference
\end{itemize}
\columnbreak
\begin{itemize}[noitemsep]
    \item Choice of coordinate frame is arbitrary
    \item[$\implies$] Shouldn't affect our inference
\end{itemize}
\end{multicols}
\vspace{-\baselineskip}
% This choice of basis is arbitrary, and shouldn't affect our inference. The same is true of the choice of coordinate system, and this property is well studied as \textit{stationary} stochastic processes. This work can be seen as extending the concept of stationarity to $R^n$ and vector valued functions.
The is strongly related to the physical principle of the \textbf{homogeneity of space} and the symmetry of natural laws.
 
\tcblower

\includegraphics[width=\linewidth]{Pictures/illustrations/change_of_gauge}
\captionof{figure}{A change of basis and coordinate system changes how we represent the location and value of a vector.}

==> poster_sections/pictures.tex <==
\includegraphics[width = 0.5\linewidth]{Pictures/feature_field_demo.pdf}
\includegraphics[width=0.2\textwidth]{Pictures/illustrations/equivariant_function.pdf}


==> poster_sections/steerable_cnp.tex <==
Neural Processes are \textit{approximations} to stochastic processes. They directly learn an approximate posterior map $Q_Z \approx P_Z$, implicitly learning a prior from data
\\[1em]
Building on proposition 1, we should ensure this approximation is \textit{equivariant}.
\\[1em]
Conditional Neural Process models learn the marginals of each location, in this case a Gaussian marginal, parametrised by mean and covariance functions.
\begin{align*}
    Q_Z = \N(\mu_Z(x), \Sigma_Z(x))
\end{align*}

To ensure this approximation is equivariant, we need the mean and covariance maps to be equivariant
\begin{align*}
    \mu_{g \op Z}(x) & = \rho(r) \mu_{Z}(g \op x) \quad
    \Sigma_{g \op Z}(x) = \rho(r) \Sigma_{Z}(g \op x) \rho(r)\inv
\end{align*}
\includegraphics[width=\linewidth]{Pictures/Equiv_CNP_flow.pdf}
\vspace{-2.5em}

==> poster_sections/stochastic_process_conditions.tex <==
% \begin{wrapfigure}{r}{0.3\textwidth}
% \begin{center}
%     % \vspace{-1.5em}
%     \includegraphics[width=0.3\textwidth]{Pictures/illustrations/equivariant_function.pdf}
% \end{center}
% \end{wrapfigure}
If we have a stochastic process $F \sim P$, the we can define the transform stochastic process $g\op P$ as the distribution of $g\op F$.
\\[1em]
Write the posterior map conditioned on some observations $Z = \{ (x_i, y_i) \}_{i=1}^n$ as $Z \mapsto P_Z$
\\[1em]
Two natural implications of the independance from coordinate systems and bases:
\begin{itemize}[noitemsep]
    \item[$\blacktriangleright$] The \textit{prior} should be \textit{invariant}, $g \op P = P \;\forall g \in \grp$
    \item[$\blacktriangleright$] The \textit{posterior map} should be \textit{equivariant}, $P_{g \op Z} = g \op P_Z \;\forall g \in \grp$
\end{itemize}
\vspace{-1.7em}
\begin{center}
    \includegraphics[width=0.42\textwidth]{Pictures/illustrations/equivariant_function.pdf}
\end{center}
\vspace{-2.8em}

% \begin{tcolorbox}
%     \begin{restatable}{proposition}{invprior}
%     \label{prop:homg_space}
%     \begin{align}
%         g \op P = P \; \forall g\in G \iff P_{g.Z}=g.P_{Z} \; \forall g\in G
%     \end{align}
%     \end{restatable}
% \end{tcolorbox}

\begin{proposition}{}{}
    \begin{align}
    \text{Invariant Prior} & \iff \text{Equivariant Posterior Map} \\
        g \op P = P \; \forall g\in G &\iff P_{g.Z}=g.P_{Z} \; \forall g\in G
    \end{align}
\end{proposition}



==> poster_sections/transforming_fields.tex <==
Changes of coordinate system in $\R^n$ form a group, the Euclidean group $E(n)$. Every element can be written as
\begin{align*}
    g = tr,  \quad g \in E(n), \; t \in T(n) \; r \in SO(n)
\end{align*}
Changes of basis (for orthogonal, same-handed bases) on $\R^n$ also form a group, $SO(n)$.
\begin{itemize}
    \item[$\blacktriangleright$] Scalar functions, $f: \R^n \to \R $, transform like
        \begin{align*}
            g \op f(x) = f(g\inv \op x)
        \end{align*}
    % \vspace{0.005em}
    \item[$\blacktriangleright$] Vector valued functions transform like
        \begin{align*}
            g \op f(x) = \rho(r) f(g \inv \op x) \quad \text{for } g = tr
        \end{align*}
        \begin{center}
            \vspace{-1em}
            with
            \vspace{-1.5em}
        \end{center}
        \begin{align*}
            \rho: \grp \to \R^{d\times d} \quad \rho(g_1)\rho(g_2)  = \rho(g_1 \op g_2)
        \end{align*}
\end{itemize}
\vspace{-1.5em}
\begin{center}
\includegraphics[width = 0.7\linewidth]{Pictures/feature_field_demo.pdf}
\end{center}
\vspace{-3em}
